Flow Splitting with Fate Sharing in a Next Generation Transport Services Architecture

The challenges of optimizing end-to-end performance over diverse Internet paths has driven widespread adoption of in-path optimizers, which can destructively interfere with TCP's end-to-end semantics and with each other, and are incompatible with end-to-end IPsec. We identify the architectural cause of these conflicts and resolve them in Tng, an experimental next-generation transport services architecture, by factoring congestion control from end-to-end semantic functions. Through a technique we call "queue sharing", Tng enables in-path devices to interpose on, split, and optimize congestion controlled flows without affecting or seeing the end-to-end content riding these flows. Simulations show that Tng's decoupling cleanly addresses several common performance problems, such as communication over lossy wireless links and reduction of buffering-induced latency on residential links. A working prototype and several incremental deployment paths suggest Tng's practicality.

==> addr.tex <==
\subsection{Factoring Addressing from Transport}

% XXX change this into "Architectural Considerations" section,
% add intro summary

The architectural motivation for factoring out the Demux layer from
the Transport layer boils down to a desire to separate issues of {\em
  endpoint addressing} from issues of {\em communication semantics}.
The Internet's network layer (IP) traditionally provides only one IP
address per host or per physical network interface, leaving a
pragmatic need for a finer-grained addressing mechanism that can
distinguish between different applications co-existing on one host.
Internet transports traditionally fill this need with 16-bit port
numbers that, when paired with an IP address, yield a logical {\em
  endpoint}.  In unicast communication, two (address, port) endpoint
pairs represent a communication {\em session}.  By embedding this
endpoint addressing function in the transport, however, this component
of the Internet's address architecture becomes conflated with the
communication semantics implemented by individual transport protocols.

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{addr.eps}
\caption{Separating Addressing Concerns from Communication Semantics}
\label{fig-addr}
\end{figure}

Factoring out port numbers and logical endpoint addressing from the
transport more cleanly separates concerns of addressing from those of
communication semantics.  Figure~\ref{fig-addr} illustrates how
addressing and communication abstractions evolve over the relevant
portion of the new ``8-layer OSI architecture'':

\begin{itemize}
\item	Layers below the Network layer can address
	only the physical links connecting a node to its immediate neighbors,
	and provide only primitive best-effort packet delivery
	as their communication abstraction.

\item	The Network layer is responsible
	for raising the addressing abstraction
	to the level of transitively reachable physical hosts,
	while leaving the communication abstraction unmodified.

\item	The Demux layer further raises the addressing abstraction,
	providing a way to address multiple logical endpoints
	on one physical host,
	while again leaving the communication abstraction unmodified.

\item	Finally, the Transport layer
	leaves the addressing abstraction unmodified,
	reusing the Demux layer's logical endpoints,
	but raises the communication abstraction,
	providing convenient semantics
	to higher-level layers.
\end{itemize}

Since the Demux layer enriches the variety of (logically) reachable
addresses and ``routes'' packets to and from those logical
``addresses,'' the Demux layer might be considered part of, or an
extension to, the Network layer.  Indeed, in a ``ground-up'' redesign
of the Internet we might aspire to design a single addressing
abstraction and routing protocol that would treat logical endpoints on
a physical host merely as ``virtual hosts'' that happen to be
implemented on one physical host; in this case the Demux and Network
layers would merge into one.  But the strong pragmatic and historical
distinctions between the functions of physical routing and logical
endpoint (de-)multiplexing suggest some utility in treating the Demux
layer as architecturally separate.

In any case, the crucial point is that port numbers and endpoint
(de-)multiplexing, though historically implemented in the transport,
has much closer architectural ties to the Network layer.  After
separating out this function, transport protocols (at least for
unicast communication) have little need to know anything at all about
the structure of host addresses or logical endpoints.  A transport
devoid of Demux layer functionality can treat endpoint addresses as
opaque bit strings, passing these strings directly through from
higher-level layers on to the next lower-level layer, and become
oblivious to the address architecture in which they exist. Such a
transport could run directly over IPv4, IPv6, UDP v4 or v6, or some
other Network and Demux layer address architecture with few or no
changes.



==> api.tex <==
describe API
interface between upper and lower sections
interfaces between layers
cross-layer communication
   - ecn


==> ccr.tex <==
Another approach,
to send to the editorial track of CCR for example...


The New OSI Layer:
why transport designers should stop whining
and learn to love UDP


A new layer has appeared in the OSI stack...
it goes by the acronym of "UDP",
which has traditionally meant "User Datagram Protocol"
but perhaps might better be taken to mean "Uniform Demultiplexing Protocol".
In the old scheme, the transport layer sits on top of the network layer;
in the new Internet architecture, the transport sits atop UDP.

Several have observed that the proliferation of NATs and firewalls
have made it impossible to deploy new transport protocols on the Internet;
this is only true in the old scheme:
it is perfectly possible to deploy new transports atop UDP.
In fact, UDP fills an essential role in the network architecture
between the network and transport layers -
a role that was unrecognized in the original OSI layering model
but whose importance is made clear by recent decades of Internet evolution.

This paper is not so much proposing a change to the Internet architecture
as recognizing that _a change has occurred_,
and proposing that we recognize the technical benefits of that change
and thus learn to like it.


Important related paper:
Handley, "Why the Internet only just works"


Note:
the Internet _has_ routed around
the ossification of the old transport layer,
by creating a new and better position in the protocol stack
for the transport layer to sit.


Talk about:
- transport negotiation
- the state tracking and keepalive problem



==> endp.tex <==
\section{The Endpoint Layer}
\label{sec-endpoint}

\com{
Our architecture's {\em Endpoint Layer}
extends the Network Layer's address space
of physical hosts and network interfaces
into an address space of {\em logical endpoints},
allowing many logical endpoints to share one physical host.
We view the Endpoint Layer as an extension to the Network Layer:
where the Network Layer provides {\em inter-host addressing and routing}
via IP addresses,
the Endpoint Layer provides {\em intra-host addressing and routing}
via port numbers.
The Endpoint Layer does not otherwise affect
the underlying best-effort delivery service:
higher layers are responsible for
congestion control, ordering, and reliability.
All higher layers ideally reside atop a single Endpoint protocol,
sharing one endpoint address space per host.
}%com

This section
outlines background and motivation for \tng's Endpoint Layer,
defines its architectural role
and the immediate benefits it brings,
explores ways the Endpoint Layer's role
might evolve in the long term,
and finally discusses implementation and deployment considerations.

\xxx{ clarify: we propose two things - factoring out endpoints
	and sharing them among transports,
	and generalizing the notion of endpoints.
	Our prototype demonstrates the first;
	the second aspect we explore (briefly!) for architectural clarity
	but leave its protocol design and implementation to future work.}

\input{epbg}
\input{epdef}
\input{epattr}
\input{implep}

\com{
\input{implic}
\abbr{}{\input{myth}}
}%com

\xxx{	consider reviving ``Transport Implementation Flexibility''
	and/or ``Negotiation of Alternative Transports'' sections
	from HotNets paper? }



==> implic.tex <==
\subsection{Practical Benefits}

Independent of the concerns of Tennenhouse and Feldmeier,
factoring out endpoint multiplexing
brings several practical benefits that are relevant today:
transport implementation flexibility,
firewall/NAT traversal, and
transport protocol negotiation.

% XXX summarize?

\subsubsection{Transport Implementation Flexibility}

\xxx{move to "implementation trust" subsection}

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{kernuser1.eps}
\caption{A UDP-based user-space transport
	{\em cannot} interoperate with 
	a ``native'' IP-based kernel-space transport.}
\label{fig-kernuser1}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{kernuser2.eps}
\caption{A UDP-based user-space transport
	interoperates with
	a UDP-based kernel-space transport.}
\label{fig-kernuser2}
\end{figure}

The IP header's 8-bit Protocol field\abbr{}{~\cite{rfc791}}
was intended to distinguish between only a few standard transport protocols,
not between many application-level endpoints,
so most operating systems prohibit unprivileged applications
from ``hooking'' IP Protocol numbers
in the way they can allocate and use ports.
The OS thus reserves the right
to implement new ``first-class'' transports.
If an application wishes to deploy its own transport protocol
that is not yet supported by the host OS,
it must layer the new transport atop UDP.
The resulting application-level transport
not only has second-class status but
is {\em unable to interoperate} with a first-class OS-level implementation
of the same transport on another host,
as shown in Figure~\ref{fig-kernuser1}.
This restriction creates a barrier to the deployment of new transports,
since the easiest way to deploy new protocols incrementally
is often to bundle them with the applications that need them.

If new transports are built atop an Endpoint Layer, however,
applications can easily ship with new transports
implemented in user-space libraries requiring no special
privilege. Once a transport begins migrating into OS kernels,
kernel-level and user-level implementations of the same
transport can remain interoperable, as shown in
Figure~\ref{fig-kernuser2}. 

\abbr{}{We note that leaving transports in
user-space is one natural consequence of our architecture, which
allows for more parallelism and performance optimizations by pushing
packet processing out of the kernel context~\cite{netchannels}.}

\subsubsection{Transport-Independent Middlebox Traversal}

\xxx{I think this section is being subsumed above.}

For better or worse,
{\em middleboxes} such as firewalls
and network address translators (NATs)
\abbr{}{~\cite{rfc3022}}
are now ubiquitous,
and most of them are sensitive to
the full endpoints of a given flow:
not only IP addresses but port numbers as well.
Since each transport traditionally implements its own port space,
middleboxes must parse transport headers,
and so only the few already-ubiquitous transports---TCP and UDP---%
can traverse most middleboxes.
New transports like
SCTP~\cite{rfc4960} and DCCP~\abcite{rfc4340}{kohler06dccp}
that are designed to run directly atop IP
thus cannot traverse most middleboxes.
NAT proliferation has in effect shifted the Internet's ``narrow waist''---%
the ubiquitous interface
atop which new protocols may be built and reliably deployed---%
upward to encompass not just IP but also TCP and UDP~\cite{rosenberg08udp}.

By building new transports atop a shared Endpoint Layer, middleboxes
need to understand only Endpoint Layer and
not Transport Layer headers.  Middleboxes can still recognize and
optimize the handling of specific transport protocols
%(operating atop the Endpoint Layer),
if desired, but doing so is no longer a
{\em prerequisite} for traversal.
The Endpoint Layer also provides a clean space for mechanisms 
allowing hosts to ``advertise'' endpoints
intended to be publicly reachable,
enabling middleboxes to create persistent bindings for them
as policy permits---%
a demand currently met via ad hoc, transport-specific mechanisms
such as those in
UPnP~\cite{upnp01igd}\abbr{}{ and NAT-PMP~\cite{cheshire05nat}}.

\com{By building new transports atop a shared Endpoint Layer,
middleboxes need not understand or modify transport layer headers.
If we take UDP as our initial Endpoint Layer protocol,
any new transport built atop UDP gains the ability to traverse
the majority of deployed middleboxes.
Middleboxes can still recognize and optimize the handling of
specific transport protocols (operating atop UDP), if desired,
but doing so is no longer a prerequisite for {\em any} traversal.

UDP tunneling has long been used for NAT traversal~\cite{
	rfc3519,rfc3947,rfc3948,rfc4380},
but UDP-based variants of transports such as SCTP and DCCP~\cite{
	ong00tunneling,tuexen07udp,phelan08datagram,denis08udp}
encounter resistance because this design conflicts
with the traditional architectural model.
In our view,
building transports atop an Endpoint Layer protocol such as UDP
{\em is} the architecturally sound approach,
yielding benefits beyond the special case of NAT traversal;
we see transports built atop IP
merely as a historical legacy.
}

\subsubsection{Negotiation of Alternative Transports}

\xxx{move to protocol design/implementation section?
	because this only necessarily applies
	to the use of UDP as our endpoint layer;
	a new endpoint layer could include or exclude a "transport tag"
	from an endpoint identifier however we see fit.}

Many application protocols
such as RPC\abbr{}{~\cite{rfc1831}} and SIP\abbr{}{~\cite{rfc3261}}
can use several alternative transports.
Every application packet is traditionally associated
with {\em exactly one} transport protocol, however,
via the IP header's Protocol field.
Negotiating {\em which} transport to use for a communication session
therefore requires the initiating application either to use
a special transport exchange just for this negotiation,
or to open new sessions ``speculatively'' for each supported transport,
only to continue using the most preferred one that succeeds
and shut down the rest.

\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{nego.eps}
\caption{Applications can negotiate among several UDP-based transports
	with no extra round trips.}
\label{fig-nego}
\end{figure}

Building transports atop a shared Endpoint Layer with one port space,
in contrast,
leaves transport identification and negotiation
under the application's control.
The Internet already follows this design philosophy
for Session Layer and Presentation Layer functions,
leaving their negotiation up to applications
(e.g., HTTP's persistent streams and content encodings\abbr{}{~\cite{rfc2616}});
our architecture extends this flexibility
to the Transport Layer.

Without prescribing specific mechanisms,
we suggest one way an application in our model
might combine transport negotiation
with the initial exchange of the selected transport,
avoiding unnecessary round-trips or state setup.
The application first locally requests from each supported transport
a copy of the ``SYN'' packet the transport {\em would} send
to initiate a new session.
The application collects the SYN packets
for all such transports,
bundles them together into one ``Meta-SYN'' packet,
and sends the Meta-SYN to the responding endpoint,
as shown in Figure~\ref{fig-nego}.
The responding application breaks apart the Meta-SYN,
passes the SYN for some transport it supports
to its implementation of that transport,
and subsequent communication proceeds normally via that transport.
This design assumes that packets for different transports
are distinguishable from each other and from Meta-SYN packets;
the application might interpose a minimal header for this purpose if required.

A side effect of
making endpoints transport-independent
is to close the debate over whether
to allocate well-known ports across several transports at once.
IANA would need to manage only one port space,
and existing applications could adopt new transports
without having to register new ports for each.

\com{
\subsubsection{Administrative Simplicity}

IANA currently manages a well-known port space
for each transport protocol,
and there is ongoing debate on whether to allocate new well-known ports
across several transports at once
or only for those transport(s)
the application already supports~\cite{cotton08iana}.
Building transports atop a common Endpoint Layer
reduces the number of port spaces IANA must manage to one,
and eliminates the allocation policy question entirely.
}

\com{
  XXX A ``tower of SAPs'' is bad for high-performance implementations,
  because when each layer has its own little address component,
  you have no choice but to dispatch each component separately.
  With one big endpoint-address, you can dispatch it all at once
  to a specialized, integrated-layer path that was formed at negotiation time.
  (XXX ref x-kernel?)
}



==> impliso.tex <==
\subsection{Implementation Considerations}

The Isolation Layer
is the first truly ``end-to-end'' layer in our architecture,
and its primary function
is to enforce this ``end-to-endness''
by cryptographically protecting the communication channel
from eavesdropping or interposition (``man-in-the-middle attacks'').
The Isolation Layer is also responsible for separating
the application's notion of host identity from the network's,
if appropriate.

These services could be implemented using existing protocols
such as IPsec or HIP, or a combination of the two:
IPsec provides authentication and privacy protection,
but not locator/identifier separation;
HIP provides locator/identifier separation and authentication
but not privacy protection.  \xxx{VERIFY!}


==> implsem.tex <==
\subsection{Implementation Considerations}

Finally, new Transport Layer protocols will build upon the Flow Layer to offer 
communication abstractions such as 
reliable byte streams \cite{rfc793}, 
reliable datagrams \cite{rfc1151}, 
media frames \cite{rfc3550},
multi-streams \cite{rfc4960}, or
structured streams \cite{ford07structured}.
We need to consider how to reposition transports
atop the Flow Layer in an incremental and backward-compatible way,
and how the absence of congestion control in the Transport Layer
may impact transport mechanisms
such as (fast) retransmit and receive window control.




==> iso.tex <==
\section{The Isolation Layer}
\label{sec-iso}

Having factored out network-oriented transport functions
into the Endpoint and Flow Layers,
we finally have a place in the layering model
where functions that isolate the application from the network,
such as location independence and security mechanisms,
cleanly fit.
We first review relevant background,
then specify the role and scope of the Isolation Layer in our model,
and finally discuss implementation considerations.

\subsection{Background: Where to Put Security?}

%Since strong security was not designed into TCP/IP,
%it had to be incorporated after-the-fact.
%For ease of implementation and deployment
%the natural approach was to insert it as a new layer
%somewhere in the protocol stack---but where?

IPsec~\cite{rfc4301},
authenticating and encrypting packets
between the Network and Transport Layers,
operates transparently with existing transports and applications
once the end hosts' operating systems are correctly configured.
However, IPsec cannot easily be deployed with or managed by applications
such as web browsers,
because implementing or interposing on transport (and below) protocols
usually requires administrator privileges and kernel extensions.
Since widely deployed NATs and firewalls
see raw IPsec packets as those of an unknown ``transport'' and filter them,
IPsec's usefulness for end-to-end security have diminished
to filling the niche of implementing Virtual Private Networks (VPNs)
by operating in tunnel mode with UDP encapsulation~\cite{rfc3948}\footnote{
	Though IPsec supports UDP encapsulation in Transport Mode,
	it requires the IPsec implementation to adjust
	the encapsulated transport headers on decryption
	according to changes made to the IP/UDP headers by NATs, thereby
	defeating IPsec's primary benefit of transport-independence.}
IPsec also interferes with performance enhancing proxies,
as described in Section~\ref{sec-bg}.

The SSL/TLS approach~\cite{rfc4346}
of authenticating and encrypting above the Transport Layer
but just below the application,
on the other hand,
is easy to implement and deploy in a library linked with applications,
and is widely used for secure Web browsing.
However, since TLS generally requires the application to manage keys itself
and negotiate a new security context for each transport instance,
many applications still use unsecured transport connections
because of the complexity of managing keys
and the performance costs of negotiating TLS connections~\cite{
	apostolopoulos99transport,coarfa06performance}.
Furthermore,
since TLS must run atop whatever transport abstraction the application chooses,
securing a transport with different semantics
than the one TLS was originally designed for---the reliable 
bytestream abstraction---
requires modifying TLS~\cite{rfc4347}.

\subsection{Defining the Isolation Layer}

We believe that the tension between the IPsec and TLS approaches 
exists
because the only suitable place for security
is {\em in the middle of TCP},
above TCP's network-oriented functions
but below its application-oriented functions.
The basic purpose of communication security is to enforce an isolation barrier
between the application and the network,
preventing devices in the network path
from either eavesdropping or interposing on
the application's end-to-end communication.
Placing end-to-end security below any network-oriented functions
denies the network the necessary ability to interact with those functions,
as we observe from IPsec's incompatibility
with middleboxes.
Placing end-to-end security above any application-oriented functions
exposes those functions to attack---
enabling devices in the network to interfere
with the transport's end-to-end reliability for example---
and entangles the security mechanism with transport semantics
so that it must be modified afresh for each new transport.
Our Isolation Layer therefore places security
exactly at the boundary
between network-oriented and application-oriented functions,
providing maximal protection for arbitrary transports
while permitting the network to interact with network-oriented functions
such as endpoint identity and congestion control.

Our Isolation Layer is also correctly placed
for isolating the application's notion of endpoint identity
from that of the network.
%The overloaded use of IP addresses
%for the purposes of network-level routing and application-level naming~\cite{
%	saltzer82naming}
%causes many difficulties,
%especially for mobile or dynamically-addressed hosts.
%There is a widespread desire to separate these functions
%so that hosts can change network-level addresses
%while retaining stable application-level identities.
Protocols such as HIP~\cite{rfc4423} and UIA~\cite{ford06persistent}
insert a layer between the Network and Transport Layers,
much like IPsec does,
this time to transform not the {\em data} the application transmits
but the {\em addresses} it uses to indicate a desired communication peer.
Instead of using network-level IP addresses directly,
applications atop UIP or UIA name other hosts via
self-certifying cryptographic identifiers keyed to the target host~\cite{
	mazieres99separating};
the interposed ``address isolation'' mechanism
translates this cryptographic identifier to a routable network-level address
and re-evaluates this mapping
whenever either participant changes network location.
If this transformation occurs below any network-oriented functions,
however,
then those network-oriented functions must operate on addresses
that are meaningless to the network,
and the transformation layer interferes with middleboxes
in the same way that IPsec does.
If this transformation occurs above any network-oriented semantic functions,
then those functions are exposed to raw network addresses,
breaking the transport's end-to-end semantics
whenever network addressing or connectivity changes.
Thus, we believe that our Isolation Layer
represents the appropriate place to implement address isolation mechanisms
like HIP.

\input{impliso}

\xxx{

The Isolation Layer in our architecture
demarks and enforces the boundary
between the network-oriented functions
implemented by the Endpoint and Flow Layers,
and the application-oriented functions
implemented by the Semantic Layer.

With the network-oriented transport functions
factored out into the Endpoint and Flow Layers,
we 

The Isolation Layer demarks and enforces the boundary
at which network concerns and application concerns begin.


XXX key points:
- represents the functionality provided by both HIP and IPsec.
- strong security requires strong identification of the principals
who are communicating;
this strong identification is also key to providing
secure location-independence.
- isolation layer is inherently a deliberately-imposed ``wall''
across which information flow is severely restricted;
thus it is important to place that wall correctly.
We believe the correct placement is above ``network-facing''
but below ``application-facing'' functions,
because in-network mechanisms have legitimate needs
to see and interact with network-facing mechanisms and protocol headers,
whereas visibility into application-facing mechanisms
would be an inherent security vulnerability at least in terms of privacy
because the application is what's supposedly being privacy-protected.
Example: bad interactions between ECN and IPsec, etc.



Identity layer provides separation point between network-oriented
identity and user-oriented identity. 
\xxx{clarify: between low-level identifiers that are efficient
for routing and regulating network traffic,
and high-level identifiers that are useful to applications and users.}

The Identity Layer is the point of separation between network-oriented
addressing, tagging, and routing below, and user-oriented addressing
and routing above. The Endpoint Layer provides network-oriented
addressing, with an evolution to incorporate tags that allow flow
terminators regulate flows (at the Flow Layer) based on scopes such as
user/group ids, that are different than IP address and port
number. 

The Identity Layer maps from these endpoint addresses to user
identities, giving the Transport Layer above it a single identity to
bind to. In the simplest case, user-level identities can be the same
as network-oriented ones, as in the current Internet where IP address
and port number provide the only clue to identity that can be used by
an application. In the general sense that we envision it however, the
Identity Layer can provide a mapping from user identity to network
location, and is the layer where functionality such as user-level
authentication/security and policy can be implemented.

HIP, SIP, shim6, i3, TRIAD, UIA, and Skype are examples of protocols
and/or architectures that approximately implement the functionality of
the Identity Layer.

\xxx{important detail:
layers above the Identity layer should be
as oblivious as possible to identity/address architecture.
They should treat identities/addresses
as opaque {\em variable-length} bit strings,
Variable-length is necessary to enable reuse of arbitrary 
existing identity namespaces,
such as Skype IDs;
and because some useful identity namespaces are cryptographic,
and cryptographic values need to increase in size over time
as both crypto algorithms and attacks on them evolve.}



Historical:

IPsec was originally intended as a general-purpose security mechanism
for the Internet,
but in practice it has found widespread deployment
only for the specific purpose of corporate virtual private networks (VPNs),
losing out to SSL in particular
for purposes of securing Web and E-commerce communication.
One reason: it was not deployable at application level;
it required root privilege and sometimes kernel extensions.
Our Endpoint Layer solves that.
Another reason: because its ``principals'' are tied to IP addresses,
it understood identity only at a machine granularity,
not at a user account granularity.
But our Identity Layer allows logical identities
to be decoupled from physical routing endpoints---%
partly for location-independence,
but also so that principals used for security
can be set to administratively sensible granularity.

SSL has the big problem of being on the wrong side of the semantic layer,
so it's specific to TCP ordering/reliability semantics---%
it had to be hacked into a new protocol, DTLS~\cite{rfc4347},
in order to secure datagram-oriented transports.
And it can't operate in application-transparent fashion
like IPSEC can.

We intend our Identity/Flow layer
to be configured and deployed in either
an OS-driven or application-driven fashion.


}%xxx



==> modes.tex <==
\subsubsection{Multipath Delivery Modes}

\com{
While a multipath best-effort delivery service
may be {\em semantically} identical to single-path best-effort delivery,
its performance profile is different.
}%com
Existing transports and applications commonly assume
that packets follow a single path through the network,
%whose round-trip delay may be measured accurately,
%and in which packets are reordered only occasionally
%due to network reconfiguration events.
and perform poorly if traffic is naively distributed
among paths with varying delay~\cite{lee02improving,lim03tcp}.
On the other hand, some transports and applications
can exploit multiple paths when available~\cite{XXX}.
For compatibility with existing upper layer protocols, therefore,
a multipath delivery service must be sensitive
to the capabilities of upper layer protocols.

We distinguish between three {\em multipath delivery modes}
describing how an upper layer protocol's packets
may be distributed among multiple paths:
{\em serialized}, {\em free}, and {\em indexed}.

\com{
We propose a simple and incrementally deployable
{\em multipath discovery mechanism},
analogous to the existing path MTU discovery mechanism,
for this purpose.
Through this mechanism,
upper layers can
discover the existence of alternative Network Layer paths,
and enable their use
in one of three different ``modes'':
{\em serialized multipath}, {\em free multipath}, and {\em indexed multipath}.
}%com

\begin{itemize}
\item	%{\bf Serialized Multipath:}
%\paragraph{Serialized Multipath:}
In {\bf\em serialized multipath delivery},
the network emulates single-path routing
by preserving packet delivery order in steady-state operation:
e.g., by using only one path at a time for traffic
between a given endpoint pair~\cite{XXX},
by delaying and reordering packets at the receiver~\cite{
	chen99new,XXX},
or via order-preserving traffic dispersion~\cite{
	gustafsson97literature}.
A multipath delivery service may implement this mode transparently
without knowledge of or interaction with upper layers.

\item	%{\bf Free Multipath:}
%\paragraph{Free Multipath:}
In {\bf\em free multipath delivery},
the network may freely distribute packets individually
among multiple paths with varying delay.
The delivery service may operate in this mode
only if the upper layer indicates support.
This mode is suitable for upper layer protocols
that are insensitive to reordering and RTT variance,
such as bulk delivery protocols with ACK batching~\cite{XXX},
and protocols that measure and adapt to reordering~\cite{XXX}.

\item	%{\bf Indexed Multipath:}
%\paragraph{Indexed Multipath:}
In {\bf\em indexed multipath delivery},
the network uses multiple paths
only under the control of the upper layer.
The upper layer can maintain per-path state
and explicitly associate packets with paths.
The delivery service might indicate
a total count of available end-to-end paths to the upper layer
%between a given pair of endpoints
via a mechanism analogous to Path MTU Discovery~\cite{XXX};
the upper layer uses this count to size a per-path state table.
The upper layer assigns a {\em path index} to each packet it transmits,
each index value indicating a unique network path.
The upper layer need not be aware of the properties of each path
beyond those it can measure (e.g., delay, MTU),
and the network may use the path index
to index into multipath routing tables~\cite{XXX},
or to seed pseudorandom bit streams
used at decision points~\cite{motiwala07path}.	% XXX Flow-Aware Net?
\end{itemize}

This distinction between multipath delivery modes
is relevant at several layers in our architecture,
as we elaborate below.

\com{
This multipath discovery mechanism
is useful and relevant across several layers in our architecture:

\begin{itemize}
\item	{\bf Flow Layer:}
The Flow Layer can use indexed multipath delivery
provided by the Network Layer
to maintain a separate congestion control context for each path,
% XXX as in ... cite?
preventing the varying path delays
from confusing the congestion control algorithm,
while avoiding the loss of RTT measurement precision
inherent in reordering-tolerant schemes~\cite{XXX}.
In its performance-optimizing role,
the Flow Layer may in turn implement
an order-preserving traffic dispersion scheme
to provide serialized multipath delivery
to a multipath-oblivious legacy transport or application,
or the Flow Layer can transparently ``pass through''
the Network Layer's free or indexed multipath delivery service
to transports and applications that support these delivery modes.

\item	{\bf Transport Layer:}
Reliable transports can similarly take advantage of indexed multipath delivery
provided by the Flow Layer
to maintain separate end-to-end retransmission state for each path,
optimizing its fast retransmit mechanism independently for each path.

\item	{\bf Application Layer:}
Some applications can benefit from indexed multipath delivery
being extended all the way up to the Application Layer:
for example, to implement multiple description streaming~\cite{
	apostolopoulos02multiple}.
\end{itemize}
}%com



==> multipath.tex <==
\subsection{Multipath Communication}

Multipath communication mechanisms are employed for two primary
purposes: (i) to increase network reliability, and (ii) to enable
distribution of load over the multiple points of connectivity.  Since
multipath communication is a network-oriented functionality that has
more to do with making the best use of available network paths than
with user communication semantics, we factor it out of the transport
layer, and into our Flow Layer.

When endhosts or middleboxes are multihomed~\cite{rfc1122}, our Flow
Layer negotiates and maintains multipath sessions between the
multihomed nodes. As shown in Figure~\ref{fig-multipath}, these
multipath sessions can be end-to-end when either or both of the
endhosts are multihomed, or between multihomed Flow Layer middleboxes,
or between a multihomed middlebox and an endhost---any Flow Layer
segment can be multipath.

\com{
\begin{figure}[tbp]
\centering
\includegraphics[width=0.5\textwidth]{flow-multipath.eps}

\caption{Multipath communication at the Flow Layer for data flow from
  Host A to Host B. Multiple paths are negotiated and used when they
  are visible at the Flow Layer. In this illustration, Host B may be
  multihomed with two IP addresses, resulting in a multipath
  segment2.}

\label{fig-multipath}
\end{figure}
}%com

In the current Internet architecture, these multipath
communication-enhancement strategies can be arranged at several
layers: at the network layer~\cite{
	gustafsson97literature,		% wired - traffic dispersion
	motiwala08path,shim6,		% wired - alternate-path
	lee01split,marina01ondemand	% wireless
	}
at the transport layer~\cite{
	hsieh02ptcp, rfc4960, iyengar06concurrent,	% wired
	magalhaes01transport},				% wireless
or at an overlay layer~\cite{andersen01resilient\abbr{}{, han04overlay}}.
We now discuss our
multipath architecture in the context of these current schemes.

\subsubsection{In-network transparent multipath}

Since each Flow Layer segment can consist of several Network Layer
routing hops, any form of concurrent multipath use is likely to
introduce reordering in the upper layer sessions. This has immediate
consequences for Transport Layer reliability
mechanisms---specifically, for TCP's fast retransmission and timeout
recovery mechanisms.  The more aggressive fast retransmission
mechanism has a low degree of tolerance to reordering, and may err and
detect packets as lost when the degree of reordering is high.  A TCP
sender uses observed round-trip times and variability to predict
timeout periods for recovery from losses, and large variability in
round-trip time due to load distribution will lead to slower timeout
recovery. Further, applications that do not care for these reliability
mechanisms may still be intolerant to reordering in the network: for
instance, a voice-over-IP application with low tolerance to delay and
jitter may find reordering and the consequent delay in playback far
more intolerable than the additional bandwidth gained from the load
distribution.

These undesirable consequences have precedence in the current Internet
architecture: several in-network transparent multipath techniques have
been proposed for Network Layer routers~\cite{rfc4116,
  prasad07queueing, kodialam06versatile}. In moving this functionality
closer to the endpoints, {\em shim6} is a recent effort that, while at
the endhost, still transparently handles multihoming~\cite{shim6}, and
from the transport's and application's points of view, continues to
suffer from the same problems as any other in-network multipath
scheme. A key lesson we learn from this precedent is that the
Transport and upper layers must be able to know how these in-network
schemes have distributed the application flow's packets in the
network. Our Flow Layer informs the upper layers about Flow Layer path
diversity, about how packets are distributed in the Flow Layer
network, and allows the upper layers to control load distribution
through these paths.

Our Flow Layer provides a hook that can be used by the Transport and
upper layers to associate specific data segments with specific paths
through the network. At the sender, the Flow Layer generates and
embeds a $k$-bit nonce, called the {\em path-seed}, in each Flow Layer
packet. The path-seed is generated per-packet, and in a weak form of
source-routing based on {\em path splicing}~\cite{HOTNETS07,
  SIGCOMM08}, determines the next segment at every Flow Layer
node. Every Flow Layer node uses the path-seed to decide the next
among multiple possible next segments, if there are more than one, to
be used for this packet. Figure XXX illustrates the nonce-based load
distribution using a simple scheme at a multipath Flow Layer segment,
where all packets with even path-seeds are forwarded on one path, and
all packets with odd path-seeds are forwarded on the other path. At
the sender, the Transport Layer can communicate with the Flow Layer to
associate data segments with path-seeds and then use per-path signals
for the reliability mechanisms. For instance, the Transport Layer
would use only data that was sent on the same path as a missing packet
to trigger a fast retransmission for the missing packet.

\begin{figure}[tbp]
\centering
\includegraphics[width=0.5\textwidth]{flow-pathseeds.eps}

\caption{Load distribution at the Flow Layer using path-seed
  nonces. The sending Host A sets the path-seeds per packet at the
  Flow Layer. An interposing Flow Layer middlebox employs these
  path-seeds by sending, as an illustration, packets with even
  path-seeds on one path and packets with odd path-seeds on another
  path.}

\label{fig-pathseeds}
\end{figure}

Other methods of dealing with reordering at the ends themselves, such
as those used by RR-TCP~\cite{zhang02improving, zhang04transport},
TCP-PR~\cite{bohacek03tcppr}, and others~\cite{blanton02making} that
learn from observing reordering in the flow, can be used at the
Transport Layer instead of using path-seed information. However, even
these methods will be able to improve their performance if they can
incorporate this Flow Layer information.

\jana{Available path diversity can be determined at Flow Layer session
  setup time, with participation from the Flow Layer entities on the
  path...}  

\com{
Routing schemes employ multihoming for fault-tolerance and load
distribution that is transparent to the ends~\cite{BGP work,
  other?}. Endpoints can thus be blind to the existence of multiple
redundant paths in the network graph and let the routing
infrastructure handle the use of this redundancy. This ideal, however,
often yields suboptimal results.

The Internet's routing architecture is hierarchical, with intra-AS and
inter-AS routing as the lower and higher scales of this hierarchy. At
the inter-AS scale, BGP, the routing glue that holds the Internet
together, glosses over detailed topological information, and uses
heavily filtered and summarized intra-AS routing information. While
this hierarchy allows for the scaling that is a hallmark of the
Internet architecture, it comes at the cost of slow responsiveness to
failures in the network due to BGP's conservative resolution of
tradeoffs between responsiveness and stability. Wide-area routing
failures take long periods of time to recover, sometimes on the order
of 30 minutes~\cite{RON}. Further, BGP is a policy-driven routing
protocol, and policy can prevent BGP from choosing a physically
available alternative path when failure occurs.

Routers also employ multihoming for load distribution, so that when
multiple forwarding paths exist for a given set of destinations,
traffic load to these destinations can be distributed among these
paths~\cite{OSPF link weights, other?}. This idea is extremely
attractive in cases where the ability to randomize outgoing traffic
among multiple paths enables more balanced, and hence more
predictable, loads on those paths, resulting in better network
provisioning and performance~\cite{Marina INFOCOMM work, TV Lakshman
  work}. While load balancing enables better utilization of network
resources, this happens in-network, transparent to the endhosts, with
packet reordering being a major side-effect that has serious
consequences for end-to-end performance.

A sending (TCP-like) endpoint will use observed round-trip times and
observed variability to predict timeout periods for recovery from
losses in the end-to-end data stream. Large variability in round-trip
time measurements to the receiver due to in-network load distribution
leads to slower timeout recovery. The more aggressive fast retransmit
mechanism has a low degree of tolerance to reordering, and may err and
detect packets as lost when the degree of reordering due to in-network
load distribution is high. While TCP endpoints can be equipped to
somewhat cope with these side-effects~\cite{RR-TCP, TCP-PR}, any
in-network technique that ignores the reality that TCP endpoints are
very sensitive to reordering is unlikely to see deployment. Further,
applications that do not care for these loss detection mechanisms may
still be intolerant to reordering in the network: for instance, a
voice communication application with low bandwidth requirements (such
as Skype) will find the jitter-buffer required to handle the
in-network reordering and the consequent delay in playback far more
intolerable than the additional bandwidth gained from in-network load
distribution.

Multihomed stub networks such as campus and corporate networks that
are diversely connected via multiple ISPs employ BGP and other tricks
for multipath communication~\cite{rfc4116}. In moving this
connectivity closer to the endpoints than in the routing sublayer,
{\em shim6} is a recent effort that, while at the endhost, still
transparently handles multihoming~\cite{shim6}, and from the
application's point of view, continues to suffer from the same
problems as any other in-network multipath scheme.

\com{Campus and corporate networks are often connected to the Internet
  via different ISPs, allowing these multihomed stub networks to
  employ these connections for fault tolerance and load
  distribution. When these networks use Provider Assigned IP addresses
  for their endhosts, the network must renumber all endhosts if the
  active path fails and traffic needs to be routed through a backup
  ISP. As a consequence, application and transport sessions will fail
  over this renumbering (re-homing) as a side-effect.

  Provider Independent (PI) addressing offers some respite, and allows
  a large enough stub network to advertise its set of IP addresses
  through any of the ISPs that it is connected to. PI addressing makes
  it possible to recover from failure without a need to renumber the
  endhosts, and allowing application sessions to be retained across
  network failures. However, scaling in the number of advertised
  prefixes is a concern with increasing numbers of multihomed stub
  networks, since these PI addresses being advertised are not
  necessarily contiguous with the provider's address space, and are
  not likely to be aggregable by the service
  provider~\cite{rfc4116}.

  A resolution that is currently being pursued in the Internet for
  stub multihoming is the ``shim layer'': a transparent shim in the
  network layer at the endhosts that, somewhat similar to HIP,
  separates identity from location, and enables fault-tolerance and
  load balancing at the endpoint scale, albeit still clearly
  ``in-network'' due to its transparent property.}
}


\subsubsection{End-to-end multipath}

When multihoming is thus visible at the endhost, multipath
communication can be arranged at the transport layer and
above. Application overlays that employ multihomed nodes use multiple
Transport Layer connections for multipath at the Application
Layer~\cite{andersen02resilient}. SCTP and DCCP are multihome-aware
transport protocols that employ end-to-end multihoming for
fault-tolerance, mobility, and/or load distribution~\cite{rfc4340,
  rfc4960, iyengar06concurrent, mobile-sctp}. These transport sessions
bind to multiple network addresses at either endhost, thus allowing a
transport connection to span a set of IP addresses at each end of the
connection. Being the first end-to-end layer, the transport layer is
well-situated for multipath communication since it is the first to
detect failure anywhere in the end-to-end path. The Transport Layer
also has fine-grained path RTT, lossrate, and throughput information,
which can inform load distribution. Our architecture provides a clean
space for multipath communication not only end-to-end, but within
segments, where possible.

The use of path-seeds in our architecture provides more control to the
Transport and upper layers on the use of multipath communication
anywhere in the network. A simple pseudo-random number generator,
biased by the current throughput and/or loss estimates for the
different paths, can be used to generate the path-seed for each packet
and control load distribution. While several schemes can be used for
the generation and consumption of path-seeds, the number of bits used
in this nonce directly provides an upper bound on path diversity: with
a $k$-bit path-seed, at most $2^k$ paths can be used on the data
path. The Transport and upper layers can, based on the amount of
path-diversity that they can handle, limit the number of bits used by
the Flow Layer for any given application data stream. For legacy
Transport protocols that cannot handle reordering, the Flow Layer
defaults to $k=0$: the Flow Layer thus does not use any concurrent
multipath schemes when a legacy protocol such as TCP is being
used. Multipath-aware protocols such as CMT~\cite{iyengar06concurrent}
can employ the use of path-seeds with few modifications, and we expect
that extending legacy protocols to handle path-seeds will require
work, but is certainly tractable.


\subsubsection{An integrated multipath communications framework}

While in-network multipath schemes are designed for managing and
better utilizing network resources, and result in better network
provisioning and performance~\cite{rfc4116, prasad06queueing,
  kodialam06versatile}, they are often at odds with expectations at
the Transport and upper layers at the ends. As a resolution to this
tension, our architecture provides an integrated multipath
communications framework. The use of path-seeds in our architecture
allows for this evolutionary end-goal: network entities can utilize
redundancy appropriately without triggering side-effects at ends.

Our architecture provides an incrementally deployable clean solution
for using multipath techniques in-network. Based on application layer
service requests, our Transport layer can determine the amount of path
diversity that is manageable and limit the size of the path-seed
nonce. Flow Layer path-seeds can be used not only at Flow Layer
middleboxes, but also at Network Layer routers to determine among
multiple Network Layer next hops, as in path
splicing~\cite{motiwala07path, motiwala08path}. Pushing this idea
further up the protocol stack, path-seeds can be controlled by the
application (for instance, at an overlay node). Pushing this idea
further down, path-seeds can also be used to inform multipath choices
at the Link Layer for link aggregation~\cite{snoeren99adaptive,
  adiseshu96reliable}. This architecture enables quicker response to
changes in path conditions since the ends are often the first ones to
learn of these changes. Our architecture thus provides an integrated
multipath solution that cleanly enables both in-network, and
end-to-end multipath communication, and allows for application service
requests to be respected through the network stack.

\com{While home-users may currently be limited in their choice of diverse
connectivity at the endpoints, with increasing deployment of broadband
wireless and wireless mesh networks, users in general will have choice
in service providers for connectivity. Mobile users are already
increasingly having to choose between using connectivity through
cellular networks or through WiFi hotspots.

When multihoming is thus visible at the endhost, multipath
communication can be arranged at the transport layer and above.  SCTP
and DCCP are multihome-aware transport protocols that employ
end-to-end multihoming for fault-tolerance, mobility, and/or load
distribution~\cite{rfc4340, rfc4960, iyengar06concurrent,
  mobile-sctp}. These transport sessions bind to multiple network
addresses at either endhost, thus allowing a transport connection to
span a set of IP addresses at each end of the connection. Being the
first end-to-end layer, the transport layer is well-situated for
multipath communication since it is the first to detect failure
anywhere in the end-to-end path, and has fine-grained path RTT,
lossrate, and throughput information. 

The transport layer endpoints, however are not aware of the actual
routes through the network, and whether the paths share any bottleneck
links. Since fairness in the current Internet architecture is arranged
at the transport layer, a conflict appears between multipath
communication and our nominal notion of flow-rate fairness (or
TCP-friendliness). A transport connection that use multiple paths for
concurrent multipath transfer risks being too aggressive at a shared
bottleneck. On the other hand, if this transport layer conservatively
{\em assumes} a shared bottleneck, then it risks performance
degradation in the presence of independent bottlenecks due to mixed
congestion signals~\cite{AkellaICNP}. Application overlays that route
over multiple TCP hops suffer from the same problems of fairness, and
further, when these overlays are not working in tandem with the
underlying Internet routing infrastructure, their interactions can
yield suboptimal results.}

\com{An endhost is multihomed when it is reachable via multiple network
  addresses~\cite{rfc1122}. A multihomed endhost can use the multiple
  resultant paths for increased reliability and for load
  distribution. These multipath communication-enhancement strategies
  can be arranged at several layers: at the network layer for using
  multiple redundant routes through the network graph~\cite{splicing,
    shim6}, or at the transport layer (or above) for end-to-end fault
  tolerance, mobility, and/or load distribution~\cite{rfc4340,
    rfc4960, iyengar06concurrent}. While the network layer solutions
  are meant to be transparent from the upper layers' points of view,
  end-to-end solutions that require transport layer support are faster
  in responding to any failures in the end-to-end paths, and are
  better equipped to deal with the side-effects of reordering.

---
Since multihoming is a network-oriented functionality
that has more to do with making the best use of available network
paths than with user communication semantics, we factor it out of the
transport layer, and into our Flow Layer.

Our Flow Layer enables host multihoming support for reliability and
load distribution on a segment-by-segment basis (end-to-end, when
there are no interposers).

\xxx{ transports that do vs don't need per-path state:
	contrast two methods of determining when to retransmit...
	cite path splicing wrt path seeds.
	for "go wild" approach: side rrtcp, prtcp}

\xxx{ to implement in flow protocol, e.g., DCCP:
	extensions to include max paths negotiation, per-packet path seeds }

Two sequence spaces: one at flow layer, one at transport layer.

If transport wants to support concurrent multipath, to retransmit, it
should know something about scheduling of data. Default: Use single
path. Otherwise, 

1/ transport tells flow layer that it can support upto k paths,
endhost flow layer generates random logk bit nonce that seeds
decisions at each flow layer hop. Transport layer maintains path state
for endpoint:nonce combinations.

2/ transport says go ahead and do any amount of concurrent multipath,
and handles reordering through schemes such as
RR-TCP~\cite{zhang04transport}, TCP-PR.
}



==> myth.tex <==
\subsection{Concerns With the Endpoint Layer}

Several likely objections to making transports UDP-based are easily addressed.
Some may argue that transports need to be implemented in
the kernel for efficiency reasons, but a UDP-transport can be
implemented in the kernel as easily as an IP-based transport.  Some
may be concerned about the 8-byte-per-packet overhead of the UDP
header, but if if a UDP-based design eliminates port number fields (4
bytes) and payload checksum (2 bytes) from the transport-layer header,
then the effective cost is only 2 bytes.  Some may worry about the
processing cost of ``an extra layer,'' but this layering can easily be
collapsed in the implementation if needed via integrated layer
processing~\cite{clark90architectural}.  Some transports may not want
UDP's full-payload checksums, but those transports can switch to
UDP-Lite~\cite{rfc3828} when the endpoints and network path supports
it.

\xxx{
The cost of keepalive traffic to maintain long-lived UDP-based
connections across middleboxes is a concern for low-bandwidth and
power-constrained devices, but this cost can be limited through
techniques described in Section~\ref{sec-keepalive}.
}


\com{

only the kernel should be able to implement a transport,
for security reasons.
A: the only security reason that makes any sense is congestion control,
and that type of security no longer works
now that most people control their own machines.

Kernel-implemented transports are more efficient.
A: if that's true, you can implement a UDP-based transport
just as well in the kernel.

Extra layers are inefficient.
A: integrated layer processing.  If you really care,
in a particular protocol stack you can easily
integrate the UDP implementation
into the kernel-space transport implementation.

Increases the per-packet size (by eight bytes).
A: no - if the transport doesn't reimplement ports, then only 4;
if the transport also doesn't reimplement the checksum, then only 2.

Middlebox state awareness costs, keepalive overhead
A: smarter binding timeouts


XXX

Certain technical concerns are likely to be forthcoming
from those who are unfamiliar with the Internet's layering model
as described here,
but are accustomed to thinking in terms of the old OSI layering model.
This section addresses some of these concerns.

<section title="Doesn't another layer make protocol stacks less efficient?">
<t>
The only two functions UDP performs
that may impose any nontrivial cost the protocol processing path -
port number or session lookup and checksum computation/verification -
are also performed in substantially equivalent fashion
by every other standardized Internet transport protocol
that bypasses UDP to run directly atop IP:
this applies for example to
	<xref target="RFC0793">TCP</xref>,
	<xref target="RFC1151">RDP</xref>,
	<xref target="RFC4960">SCTP</xref>, and
	<xref target="RFC4340">DCCP</xref>.
Bypassing UDP therefore does not actually provide these transports
any practical savings over running atop UDP.
</t>
</section>

<section title="What if a new transport doesn't want UDP's checksums?">
<t>
For transports and applications that wish to avoid the cost of
computing and verifying the UDP checksum on every packet,
or that wish to receive partially corrupted packets
so they can use ECC or other methods to reconstruct the payload,
<xref target="RFC3828">UDP-Lite</xref>
is available for precisely this purpose.
Since UDP-Lite reuses the same port number space as UDP
and otherwise provides the same semantics as UDP to upper-layer protocols,
it does not in effect represent another Demux layer
so much as an optimization to the existing Demux layer.
To address any deployment concerns,
transports and applications can easily be designed
to fall back on traditional UDP
in situations where either participating endpoint
does not support UDP-Lite.
</t>
</section>

<!--
* Q: What if a transport needs different demultiplexing functionality?
A: It is possible that a transport might wish to present
a different "logical endpoint" abstraction to the application
than the standard one consisting of an IP address and port number,
XXX...  (maybe this question not needed...)
-->

<section title="Isn't it more efficient for a NAT or firewall to use
	protocol-specific logic to track and manage transport-layer sessions?">
<t>
It's true that middleboxes such as NATs and firewalls
can maintain their state more intelligently when they can, for example,
track the lifetime of transport-level connections
as they can with TCP.
But running a transport atop UDP in no way prevents middleboxes
from looking inside the UDP packets
and handling particular transports intelligently.
Running the transport atop UDP
merely ensures that the transport won't stop working AT ALL
over middleboxes that don't have this transport-specific intelligence.
</t>
</section>

<section title="Isn't UDP's port space too small
		to share among all transports?">
<t>
Given that transports widely deployed atop IP currently number
between two and four depending on whom you believe,
maintaining a separate namespace for each transport
effectively adds at most about two bits to the size of the port namespace.
If a 16-bit unified port space is too small, therefore,
then 16-bit transport-specific port spaces are also probably too small
or will be soon,
especially given IANA's historical policy of reserving application port numbers
across multiple transports at once.
If the size of port numbers is an issue,
the proper fix is to introduce a Demux layer extension
providing port numbers of at least 32 bits.
</t>
</section>

<section title="How can an application support multiple alternative transports
		if all these transports must run atop UDP?">
<t>
The technically simple but ultimately wrong answer
to this question
is simply to allocate a different port number
for each combination of application and transport protocol,
analogous to the separate port numbers reserved
for "plain" versus "secure" HTTP.
This solution is less than ideal because,
even discounting concerns over crowding UDP's 16-bit port space,
it requires an application supporting N different transports
to send N separate "INIT" packets - one for each transport -
to a peer with which it wishes to communicate
in order to determine which transport(s) the peer supports.
Note that transports running directly atop IP
also present this problem to applications,
while giving the application no way of fixing it.
</t>

<t>
A far better solution,
which becomes possible only when transports share a single Demux layer,
is for the application itself
to take charge of negotiating the transport protocol
it uses over a particular Demux-layer session.
The initiating application could for example request from each transport
a copy of the "INIT" packet
the transport would transmit in order to start a new connection,
and bundle all of these transport-layer INITs together
into a single application-layer "INIT bundle" packet.
Upon receiving this INIT bundle,
the responding application extracts the appropriate INIT
for some transport that it supports as well,
and hands the INIT to the selected transport protocol,
so that only the chosen transport ever responds
to the initiator's (single) INIT bundle.
Viewing the transport as "subservient" to the application in this way
both conserves port number space
and increases the efficiency of transport negotiation
for applications that wish to support multiple transports.
</t>

}%com


